FlexiRepair: Transparent Program Repair with Generic Patches

Template-based program repair research is in need for a common ground to express fix patterns in a standard and reusable manner. We propose to build on the concept of generic patch (also known as semantic patch), which is widely used in the Linux community to automate code evolution. We advocate that generic patches could provide at the same time a unified representation and a specification for fix patterns. Generic patches are indeed formally defined, and there exists a robust, industry-adapted, and extensible engine that processes generic patches to perform control-flow code matching and automatically generates concretes patches based on the specified change operations. In this paper, we present the design and implementation of a repair framework, FLEXIREPAIR, that explores generic patches as the core concept. In particular, we show how concretely generic patches can be inferred and applied in a pipeline of Automated Program Repair (APR). With FLEXIREPAIR, we address an urgent challenge in the template-based APR community to separate implementation details from actual scientific contributions by providing an open, transparent and flexible repair pipeline on top of which all advancements in terms of efficiency, efficacy and usability can be measured and assessed rigorously. Furthermore, because the underlying tools and concepts have already been accepted by a wide practitioner community, we expect FLEXIREPAIR's adoption by industry to be facilitated. Preliminary experiments with a prototype FLEXIREPAIR on the IntroClass and CodeFlaws benchmarks suggest that it already constitutes a solid baseline with comparable performance to some of the state of the art.

==> discussion.tex <==
\section{Discussion}
\label{sec.discussion}

% Donor code

% Many APR tools rely on the assumption that code fixes can be composed from the existing code bases. The question lies where to look for such code. This is a fundamental question that underpins the basic assumption of such APR tools, many reusing code from the given program's codebase (whether it's the program itself, it's history or test cases) they are trying to repair. The study shows that in 44\% of cases code from other projects would have had to be sourced.

% current program repair tools mostly fix simple bugs and generally effective if the donor code is present around the bug location.

% ) existing repair tools fix mostly simple bugs but some of the generated patches are complex. ii) most repair tools target local donor codes. iii) and finally, "When considering a large donor code search space, it is possible to fix more bugs for APR systems, but the trade-off [35] between the repair performance in terms of the number of fixing bugs and the efficiency in terms of the time cost or patch precision should be carefully maintained by practitioners to boost APR."

% Finding (iii) is a well-known fact in the program repair community. That's why each program repair tool targets a subset of bug-fixes so that it does not blow up the search space. For example, some repair techniques restrict their search to only the buggy files, some techniques apply edit operations in one location, and some techniques target a specific kind of repair such as repairing control-flow related bugs, and so on. Researchers are also learning how to gradually increase the scope that provides the best gain while keeping the search space affordable


% how can we search for repair ingredients? Such questions are particularly acute
% for generate-and-validate APR systems where defining the location
% scope of the repair ingredients can have a substantial impact on
% the quality of the patch candidates. The search space in APR patch generation is indeed determined mainly by two types of ingredients:
% the change action and the donor code.

% APR systems are generally more effective when donor code is available in the buggy program and when it is near from the bug location. There should be a higher probability to fix when exploring a larger search space but it takes more time and cost before finding successful patches.


% Finding relevant donor code is
% 209 210 211
% thus a challenging endeavour in program repair. Unfortunately, 212
% 213
% this challenge can be hidden as an engineering detail, and is thus scarcely discussed in the literature. APR research however must 215
% strike a good balance between efficiency (i.e., the search space must
% not explode by considering all possibilities) and effectiveness (i.e.,
% 214
% 216 217 218
% the search space must include the relevant donor code to yield 219
% correct patches)

% However, enlarging the search space of
% donor code will sharply enlarge the search space of patch candidates
% hat will further increase the possibility of generating plausible but
% 1201
% 1202 incorrect patches before the correct ones [55]

==> tables/intro.tex <==
% \begin{tabular}{lllllrrr}
% \toprule
%     project & LOC & \# bb & \# wb &\# bugs & \toolname & SearchRepair & SOSRepair \\
% \midrule
%   checksum & 13 & 6 &   29  & 23 &     23 & 0  & 3\\
%      digits & 15 & 6 &   91  & 37 &   8   & 0  &24\\
%       grade & 19 & 9 &   226 & 12 &  8  & 2  &37\\
%      median & 24 & 7 &   168 & 44 &  27  & 68 &87\\
%   smallest & 20 & 8 &   155 & 75 &  56  & 73 &120\\
%   syllables & 23 & 6 &   109 & 70 &  64  & 4  &75\\
% \bottomrule
% total    &   114 & 42 & 261 & 778 & 186 & 150 & 346
% \end{tabular}


\begin{tabular}{l|rr|r|rr}
\toprule
          & \multicolumn{2}{c|}{ \# Tests} &  &  \multicolumn{2}{c}{\toolname}\\
  Project &  WB& BB & \# Bugs & WB & BB\\
\midrule
  checksum & 10 & 6 &    30 & 23 & 23 \\
    digits & 10 & 6 &    83 & 37 & 8  \\
     grade & 9 & 9 &   228 & 12 & 8  \\
    median & 6 & 7 &   164 & 44 & 27 \\
  smallest & 8 & 8 &   152 & 75 & 56 \\
 syllables & 10 & 6 &   107 & 70 & 64 \\
\bottomrule
Total    & 53 & 42 &   764 & 261 & 186 & 
\end{tabular}







==> tables/whitePatterns.tex <==
\begin{tabular}{lr}
\toprule
                                   pattern &  count \\
\midrule
\lstinputlisting{patternListings/white/expr_stmt_8_12.cocci4-prev}    &     82 \\
\lstinputlisting{patternListings/white/block_19_63.cocci0-cocci7}      &     47 \\
\lstinputlisting{patternListings/white/if_8_102.cocci0-cocci_patches} &     45 \\
\lstinputlisting{patternListings/white/function_4_32.cocci}            &     24 \\
\lstinputlisting{patternListings/white/if_stmt_8_8.cocci1}            &     14 \\
\lstinputlisting{patternListings/white/if_6_5.cocci-cocci_patches}    &      8 \\
\lstinputlisting{patternListings/white/block_content_87_25.cocci1}    &      7 \\
\lstinputlisting{patternListings/white/if_stmt_11_71.cocci}           &      5 \\
\lstinputlisting{patternListings/white/function_42_50.cocci1}          &      5 \\
\lstinputlisting{patternListings/white/for_5_3.cocci3-cocci2020-07-20_18-02-34} &      4 \\
\lstinputlisting{patternListings/white/if_4_10.cocci8-cocci7} &      4 \\
\lstinputlisting{patternListings/white/if_14_157.cocci-cocci7} &      3 \\
\lstinputlisting{patternListings/white/if_5_2.cocci3-cocci1} &      3 \\
\lstinputlisting{patternListings/white/block_19_60.cocci-cocci7} &      2 \\
\lstinputlisting{patternListings/white/block_content_13_46.cocci2} &      2 \\
\lstinputlisting{patternListings/white/if_5_2.cocci7-cocci1} &      1 \\
\lstinputlisting{patternListings/white/if_7_1.cocci3-cocci6} &      1 \\
\lstinputlisting{patternListings/white/if_7_13.cocci1-cocci1} &      1 \\
\lstinputlisting{patternListings/white/function_26_1.cocci-cocciFlaws} &      1 \\
\lstinputlisting{patternListings/white/if_stmt_10_94.cocci} &      1 \\
\lstinputlisting{patternListings/white/if_4_0.cocci26-cocci1} &      1 \\
\bottomrule
\end{tabular}
